HealthSLM-Bench: Benchmarking Small Language Models for Mobile and Wearable Healthcare Monitoring

Mobile and wearable healthcare monitoring play a vital role in facilitating timely interventions, managing chronic health conditions, and ultimately improving individuals' quality of life. Previous studies on large language models (LLMs) have highlighted their impressive generalization abilities and effectiveness in healthcare prediction tasks. However, most LLM-based healthcare solutions are cloud-based, which raises significant privacy concerns and results in increased memory usage and latency. To address these challenges, there is growing interest in compact models, Small Language Models (SLMs), which are lightweight and designed to run locally and efficiently on mobile and wearable devices. Nevertheless, how well these models perform in healthcare prediction remains largely unexplored. We systematically evaluated SLMs on health prediction tasks using zero-shot, few-shot, and instruction fine-tuning approaches, and deployed the best performing fine-tuned SLMs on mobile devices to evaluate their real-world efficiency and predictive performance in practical healthcare scenarios. Our results show that SLMs can achieve performance comparable to LLMs while offering substantial gains in efficiency and privacy. However, challenges remain, particularly in handling class imbalance and few-shot scenarios. These findings highlight SLMs, though imperfect in their current form, as a promising solution for next-generation, privacy-preserving healthcare monitoring.

==> Sections/01-introduction.tex <==
\section{Introduction}
Continuous healthcare monitoring is crucial in our daily life, as it enables early detection, timely intervention, and helps sustained well-being by tracking physiological status and related metrics from wearable devices~\cite{cdc2021, nih2020, pham2022pros,jia2024ur2m,wu2023udama}. Recent studies have explored leveraging wearable sensor data, such as Large Language models (LLMs) in the field of healthcare prediction~\cite{kim2023}, as they demonstrated comprehensive understanding and analysis capabilities on vast amounts of unstructured data. However, many state-of-the-art (SOTA) LLMs, such as GPT-3.5, GPT-4, Gemini-1.5 and Llama-3, require tens to hundreds of billions of parameters, demanding powerful hardware for training and inference~\cite{bind2024gemini}. As a result, most of them run on cloud for real-time inference. Cloud-based deployment can potentially lead to data leakage by necessitating the transfer of sensitive health data off-device~\cite{zhang2024enabling, Li2024}, such as the potential misuse of personal health information. Furthermore, their high computational and memory requirements make them expensive for continuous health monitoring.%\td{this reads like you are working on personalisation monitoring which is not true. Here I guess you mean general health applications.}

% \hj{I think we should also say we can ask questions by using llms?}

In contrast, Small Language Models (SLMs), with parameter size between 1B to 4B, offer a promising alternative for resource-constrained on-device deployment, such as smartphones, where memory, power, and connectivity are limited. By avoiding cloud inference, SLMs reduce latency and protect sensitive personal data while maintaining competitive task performance~\cite{microsoft2024phi3, tinylama2024,qwen2024qwen2, gemma2024}.%\td{ref}
However, their compact size may impose certain limitations%\td{rephrase not good english}
, and their application in the context of healthcare monitoring has yet to be validated. The prior work~\cite{Mobicom} demonstrated the feasibility of deploying SLMs on mobile device for predicting health status, such as fatigue, sleep quality, stress levels, and activity readiness, using multivariate time-series data from wearables. They achieved competitive accuracy with real-time latency and low memory footprints compared to SOTA LLMs. However, there are some severe limitations remaining: 1) The performance evaluation only from one dataset, the result lack of consistency and generalizability; 2) only zero-shot performance are reported, without demonstrating effectiveness under health-domain adaptation; 3) Efficiency was assessed on standard NLP datasets rather than real health datasets, limiting practical relevance for real healthcare applications. Therefore, our study aims to address the following research questions:
\begin{enumerate}
    \item How consistent and generalizable are SLMs when evaluated across multiple wearable health datasets?  
    \item To what extent can SLMs adapt to health-domain tasks under few-shot and instructional tuning, beyond zero-shot performance?  
    \item How efficient are SLMs when deployed on real health datasets, and can they sustain low latency and memory cost in practical healthcare scenarios?  
\end{enumerate}

%\td{These are not research questions; rather, they describe the experiments that have been conducted. Research questions should identify the specific problem you are addressing. For example, when analyzing few-shot learning, what is it that you aim to discover? }

In this paper, we conducted comprehensive evaluation on their performance after domain adaptation. Our contributions are outlined as follows:

% \textbf{LifeSnaps}~\cite{yfantidou2022lifesnaps}, \textbf{GLOBEM}~\cite{xu2023globemdatasetmultiyeardatasets} and \textbf{AW-FB}~\cite{fuller2020replication}, 

\begin{itemize}
\item We go beyond prior zero-shot evaluation and benchmarked various SLMs across different health applications using zero-shot, few-shot, and instruction fine-tuning approaches, and found that some SLMs, such as Phi-3-mini-4k, TinyLlama-1.1B, Qwen2-1.5B can surprisingly outperform health-domain finetuned LLMs - HealthAlpaca-lora-7b and HealthAlpaca-lora-13b under the same setting. %\td{LoRA}
% In suboptimal tasks, SLMs also achieve on-par accuracy compared with HealthAlpaca-13b.
% \td{the important message is that "We benchmarked various SLMs across different health applications using zero-shot, few-shot, and instruction fine-tuning approaches, and found that some LLMs can outperform xxx."}


\item We are the first to deploy and benchmark SLMs on mobile devices with 8 GB RAM memory, running inference on health datasets. The results demonstrate that SLMs maintain consistent performance with significant latency benefits, achieving over 21× faster response times, 32× faster overall process time and 5× lower CPU usage than LLMs such as Llama-2-7b.
% \item We further developed the mobile application and add new implementation to run inference on PMData dataset. Our Results show that, the computation load is heavier compare to standard NLP dataset-HotPotQA. Under this condition, SLMs behave consistently as HotPotQA with slightly higher response latency, while LLM Llama-2-7b struggled and only have the half speed of token producing. SLMs show a 21.3× latency improvement and 32.1× the total time spent on prediction. \td{here can we say 'We are the first to deploy and benchmark these SLMs on mobile devices with x RAM, running inference in real time. The results demonstrate that xxx.' also here we are talking about the general trend among methods, but not the comparison among datasets. You can give detailed discussion of the datasets in the result section. Here we only highlight the key message of methods.}
\item Our experiments also reveal two notable limitations of SLMs in health prediction tasks: (i) a tendency to collapse in few-shot prompting, producing identical outputs across tasks, and (ii) exhibit strong majority-class bias under instructional tuning with imbalanced datasets. These findings highlight important challenges for SLM deployment in healthcare.

% \item We identify the current limitations of SLMs for healthcare monitoring and outline promising directions for advancing their effectiveness in health-related applications. \td{This is not a contribution, but rather a necessary component found in almost every paper.}

\end{itemize}

% consume significantly less CPU usage, latency, and memory usage.

==> Sections/02-related_work.tex <==
\section{Related Work}
\paragraph{LLMs for health monitoring.} 
%With the rise of mobile and wearable devices, a variety of human-centered sensing signals can be continuously collected, enabling ongoing monitoring of human health in daily life. Resting heart rate, in particular, is one of the most common signals recorded by wearable sensors and widely used in health event prediction~\cite{ballinger2018deepheart, hallgrimsson2019learning, Mullick2022}. Recent studies have shown that the physical status data collected by mobile devices is strongly associated with health status~\cite{Mullick2022}. 
While traditional machine learning and deep learning methods have proven effective for analyzing wearable sensor data across a range of sensor modalities and health-related applications~\cite{ballinger2018deepheart, hallgrimsson2019learning, Mullick2022}, these models are often trained on specific datasets or tailored architectures, which limits their ability to generalize across diverse tasks and contexts~\cite{kasl2024generalizability}. In contrast, Large Language Models (LLMs) have demonstrated strong generalization capabilities and notable success in healthcare. For instance, Health-LLM~\cite{kim2024healthllm} and MultiEEG-GPT~\cite{hu2024exploring} showcase the effectiveness of leveraging pre-trained LLMs for healthcare monitoring using physiological data. Recent research also suggests that pre-trained LLMs like GPT-4 may reduce the need for extensive model tuning, as they exhibit robust zero-shot performance in medical reasoning tasks with minimal supervision~\cite{nori2023capabilities}. Additional approaches, including few-shot prompting, instruction tuning, and domain-specific fine-tuning, have been explored to further enhance performance on medical tasks~\cite{xu2024mentalllm}. Notably, PaLM2~\cite{singhal2023large} highlights the advantages of integrating various inference and adaptation strategies (such as few-shot learning and fine-tuning) for improved outcomes. More recently, applied systems like PhysioLLM~\cite{Fang2024PhysioLLM} have demonstrated that LLMs can deliver personalized health insights, underscoring their adaptability across different users and contexts. Despite these advancements, the significant computational demands of LLMs render them impractical for privacy-sensitive, real-time mobile and wearable healthcare monitoring.

%More recently, surveys and applied systems%\td{what do you mean here? if you are talking this paper why mentioning survey and applied systems} such as PhysioLLM~\cite{Fang2024PhysioLLM} emphasize how LLMs can be integrated with wearable sensor data to deliver personalized health insights without significant training efforts. %\td{Here, you mention achieving results without training efforts, which suggests greater efficiency, but then you note there is still computational overhead. Consider clarifying the message you want to convey.} Despite these advances, their computational overhead makes them impractical for privacy-sensitive, real-time mobile healthcare monitoring.


% Health-LLM~\cite{kim2024healthllm} and MultiEEG-GPT~\cite{hu2024exploring} leverages LLM capabilities for healthcare monitoring using text. LLMs for Mental health predictions~\cite{xu2024mental,zhang2024leveraging}, powered by few-shot and fine-tuned strategies, shows great promise in predicting mental health status. PaLM2~\cite{singhal2023large} demonstrated the effectiveness of LLMs by combining various strategies, achieving superior performance across different datasets in medical domains. Recent medical reasoning evaluations on GPT-4~\cite{nori2023capabilities} have demonstrated the great promise of LLMs in recognizing medical events without significant training efforts. However, all these models require significant computational resources, which is impractical for privacy-sensitive and real-time mobile healthcare monitoring. 

%LLMs for Healthcare Prediction
% \paragraph{SLMs.} \td{Let's focus on SLMs and primarily list the various types available. Discuss how these SLMs have demonstrated strong performance across a range of NLP tasks, citing relevant references. However, it remains unclear how well they perform in health prediction, particularly in high-stakes scenarios where accurate and timely predictions are crucial. Understanding their capabilities in health-related applications is especially important, especially when considering deployment on mobile and wearable devices. }Due to the significant number of parameters in LLMs, which makes it challenging to deploy them on resource-constrained devices, recent SLMs have emerged as efficient alternatives, showing competitive performance across many tasks. For instance, Microsoft’s Phi-3-mini-4k-Instruct~\cite{microsoft2024phi3mini4kinstruct}, with 3.8B parameters, is trained on a mix of synthetic and high-quality public data curated for reasoning-rich properties. TinyLlama-1.1B~\cite{tinylama2024tinyllama}, a distilled version of Llama 2, compresses to 1.1B parameters and is fine-tuned on UltraChat, a dataset of diverse synthetic dialogues. Google’s Gemma2-2B~\cite{google2024gemma2}, derived from Gemini research, achieves strong performance in text generation, summarization, and reasoning. HuggingFace’s SmolLM-1.7B~\cite{huggingfacetb2024smollm}, trained on synthetic textbooks, stories, educational Python, and web samples, provides broad domain coverage, while Qwen2-1.5B~\cite{qwen2024qwen2} delivers state-of-the-art results in coding and mathematics despite its compact size. More recently, Meta’s Llama-3.2 series~\cite{meta2024llama32modelcard} introduced lightweight variants (1B and 3B), further extending the trend of high-performing yet compact architectures suitable for edge deployment. 

\paragraph{Small Language  Models.}  
Recent SLMs have emerged as efficient alternatives to large LLMs, offering competitive performance across diverse NLP tasks while being lightweight enough for deployment on resource-constrained devices~\cite{demystifying2025, murthy2023}. For instance, Microsoft’s Phi-3-mini-4k-Instruct~\cite{microsoft2024phi3mini4kinstruct} (3.8B) is trained on a mix of synthetic and high-quality public data curated for reasoning-rich properties; TinyLlama-1.1B~\cite{tinylama2024tinyllama}, a distilled version of Llama 2, compresses to 1.1B parameters and is fine-tuned on UltraChat, a diverse synthetic dialogue dataset; Google’s Gemma2-2B~\cite{google2024gemma2}, derived from Gemini research, achieves strong performance in text generation, summarization, and reasoning; HuggingFace’s SmolLM-1.7B~\cite{huggingfacetb2024smollm}, trained on synthetic textbooks, stories, educational Python, and web samples, provides broad domain coverage; and Qwen2-1.5B~\cite{qwen2024qwen2} delivers state-of-the-art results in coding and mathematics despite its compact size. More recently, Meta’s Llama-3.2 series~\cite{meta2024llama32modelcard} introduced lightweight variants (1B and 3B), extending the trend of compact yet high-performing architectures suitable for edge deployment. Despite these advances, it remains unclear how well SLMs generalize to health prediction, particularly in high-stakes scenarios where accurate and timely predictions are crucial. 

% Understanding their capabilities in health applications is essential, especially for deployment on mobile and wearable devices.


%\td{then in the following part, we can focus on deployment.} 
% \paragraph{SLMs deployment.}Following on this momentum, MobileAIBench~\cite{murthy2023} deploy these SLMs on an real iPhone 14 and build a comprehensive framework to measure efficiency, latency, and memory consumption, and demonstrate efficiency. Most recent work~\cite{Mobicom} provided one of the initial explorations of SLMs for health event prediction on PMData~\cite{pmdata2020} under Zero-shot setting, highlighting their potential as practical and privacy-preserving alternatives to LLMs for mobile and wearable healthcare monitoring.

% Despite their promises in text based health applications, the performance of these models in mobile healthcare monitoring and their comparison to LLMs still remain largely unexplored. \td{this is not a deployment problem, but a general comparison betweeen slms and llms, move it to slms subsection.}Specifically, there has yet to be a systematic study examining how SLMs perform under different adaptation strategies (e.g., few-shot prompting, LoRA fine-tuning) and across multiple wearable health datasets. Address those gap is crucial.\td{This explains how to do it, but not why it should be done. In the related work section, it is more important to discuss the reasons behind your approach. Regarding the deployment of SLMs, it seems that there are already studies on deploying SLMs for mobile health applications. Do you have any additional motivations or new insights in your results that demonstrate how our deployment differs from existing ones? This should be something introduced here.} as it limits our understanding of their effectiveness and practicality for real-world, privacy-sensitive healthcare applications on mobile and wearable devices.

\paragraph{SLMs Deployment.}  
Following on this momentum, MobileAIBench~\cite{murthy2023} deployed SLMs on an iPhone 14 and provided a comprehensive framework to measure latency, memory consumption, and efficiency, demonstrating the feasibility of running compact models locally. Most recent work~\cite{Mobicom} investigated the use of SLMs for health event prediction on PMData~\cite{pmdata2020} under a zero-shot setting, highlighting their potential as practical and privacy-preserving alternatives to LLMs for mobile and wearable healthcare monitoring. While these studies demonstrate the promise of SLM deployment, they remain limited in scope. MobileAIBench focused on general NLP tasks rather than health-specific workloads, and the study presented at MobiCom was restricted to a single dataset under zero-shot evaluation. There is still missing a systematic understanding of how SLMs behave when deployed for real-world health applications across multiple datasets and adaptation strategies. This gap motivates our study, which evaluates SLMs under health-domain deployment scenarios and provides new insights into their effectiveness and practicality for privacy-sensitive mobile healthcare monitoring.



% Understanding the performance, resource efficiency, and privacy benefits of SLMs is crucial for evaluating their suitability for real-time, privacy-sensitive healthcare applications.

% %SLMs and On-Device Efficiency
% In contrast, Small Language Models (SLMs) with parameter counts between 1B–4B offer a compelling alternative for on-device healthcare applications. By running locally on smartphones or wearables, SLMs preserve privacy and reduce inference latency while maintaining competitive task performance. Prior work demonstrated the feasibility of deploying SLMs for predicting fatigue, stress, and sleep quality on mobile devices [10]. However, this study was limited to zero-shot evaluation on a single dataset, and efficiency was primarily measured using general NLP benchmarks rather than health-specific data, leaving the effectiveness of domain adaptation unexplored.

% To address this gap, adaptation strategies such as few-shot prompting [11] and instructional tuning [12] have been widely adopted in LLM research. Few-shot methods provide minimal supervision for in-context learning, while lightweight fine-tuning techniques such as LoRA [13] allow efficient domain alignment of compact models. Recent works like Alpaca [14] further highlight the utility of instruction–response datasets for aligning models with domain-specific tasks. Building on these advances, our work systematically benchmarks SLMs across multiple health datasets (PMData [15], GLOBEM [16], AW-FB [17]) under zero-shot, few-shot, and LoRA-tuned settings, providing the first comprehensive evaluation of SLMs for time-series healthcare prediction.

==> Sections/05-results-copy.tex <==
% Do not compile this file directly. Compile neurips_2025.tex instead.
\section{Results}


% \multirow{10}{*}{\makecell{\textbf{SLMs}\\(FS-3)}} 
% & gemma-2-2b-it   & 0.4816 & 1.6589 & 44.82 & 0.4883 & -     & -     & -     & - \\
% & Phi-3-mini-4k   & \underline{0.4114} & 1.6689 & 44.82 & \textbf{0.4515} & \underline{0.880} & \textbf{0.535} & 19.4 & 54.983 \\
% & SmolLM-1.7B     & - & - & - & - & \textbf{0.870} & 0.582 & 15.4 & 18.972 \\
% & Qwen2-1.5B      & \underline{0.4114} & 1.6756 & \textbf{51.51} & \underline{0.4615} & 0.883 & \textbf{0.535} & \underline{23.1} & 19.845 \\
% & TinyLlama-1.1B  & - & - & - & - & 2.933 & 3.043 & 14.4 & \textbf{17.902} \\
% & Llama-3.2-1B    & 0.4348 & 1.7324 & 49.83 & 0.5418 & 0.883 & \textbf{0.535} & 15.4 & \underline{18.472} \\
% & Llama-3.2-3B    & \underline{0.4114} & 1.7759 & \textbf{51.51} & 0.4682 & 1.194 & 1.117 & \textbf{24.1} & 19.270 \\
% & Phi-3.5-mini    & \underline{0.4114} & \textbf{1.4247} & \textbf{51.51} & \underline{0.4615} & 0.910 & \underline{0.548} & \textbf{24.1} & 32.941 \\
% & Qwen2.5-1.5B    & \textbf{0.3946} & \underline{1.4381} & \underline{37.12} & 0.7559 & 1.365 & 0.642 & 18.1 & \textbf{17.902} \\
% \cmidrule{2-10}
% & Mean            & 0.4224 & 1.6249 & 47.30 & 0.5184 & 1.240 & 0.942 & 19.2 & 25.036 \\
% \midrule


% As shown in Table~\ref{tab:performance}, after exposing with 5 examples, majority of tasks consistently outperformed zero-shot on PMData, GLOBEM and AW\_FB, particularly with the highest accuracy activity rose from 21.74 to 24.1 (+2.36\%) and lowest MAE of readiness decreased from 1.512 to 1.323 (-22\%). Instructional tuning further improved the 
% Qwen2-1.5B for STRS/SQ (0.411/0.462), SmolLM-1.7B for ANX (0.870), and Phi-3-mini-4k for DEP (0.555). On AW-FB, Phi-3.5-mini reaches the highest ACT (24.1) while maintaining low CAL (23.689).

% ANX by \textbf{5.9\%} (1.489 to 1.401), and DEP by \textbf{6.3\%} (1.552 to 1.454)

% As shown in Table~\ref{tab:performance}, SLMs in the zero-shot setting already demonstrated competitive performance across health prediction tasks, consistent with prior findings on PMData~\cite{Mobicom}. When provided with only five in-context examples (FS-5), performance improved markedly: average errors in stress, readiness, sleep quality, and calorie prediction were reduced, while activity classification became more accurate. Importantly, several tasks also reached new best results, with lower errors on readiness, anxiety, and calorie estimation, and higher accuracy on activity prediction. These outcomes highlight the strong adaptability of compact models to health-related time-series data when guided by even a small number of examples.

% With the 5 examples given in the FS-5 setting, several models demonstrated notable improvements. On PMData, Phi-3-mini-4k achieved better accuracy READ from 1.515 to 1.3244, while Qwen2-1.5B consistently yielded strong low STRS and SQ (0.411 and 0.462). On GLOBEM, SmolLM-1.7B reached the lowest ANX (0.870), and Phi-3-mini-4k performed best in DEP (0.555). For AW-FB, Phi-3.5-mini provided the best trade-off, reaching the top ACT score (24.1) while maintaining relatively low CAL (23.689).

% Under LoRA adaptation, lightweight SLMs further strengthened their performance. On PMData, TinyLlama-1.1B achieved the highest FATG (63.2) while also maintaining the lowest STRS (0.395). On AW-FB, gemma-2-2b-it reached the highest ACT (34.4) with an exceptionally low CAL (2.802), indicating strong efficiency. Overall, Phi-3-mini-4k and TinyLlama-1.1B emerge as the most balanced SLMs, consistently rivaling or surpassing larger LLM baselines such as HealthAlpaca-13B, while being far more efficient and deployment-friendly.

% For instance, The average MAE for stress prediction decreased from 0.605 to 0.422, readiness from 2.150 to 1.420, sleep quality from 0.602 to 0.470, and calorie estimation from 143.23 to 28.77, while the accuracy of activity prediction improved from 16.43 to 19.84. Best results also advanced across several tasks, with the lowest MAE for readiness reduced from 1.515 to 1.324, anxiety from 0.876 to 0.870, and calories from 19.7 to 18.581, while the highest accuracy for activity prediction increased from 21.74 to 24.1.

% SLMs are able to achieve superior performance than HealthAIpaca-lora-7b and even competitive performance than HealthAIpaca-lora-13b. For PMData, with 0.396 vs 0.34 and 0.53 in STRS, 1.304 vs 1.40 and 1.56 in READ. Similarly for FATG, SQ and other two datasets. For AW\_FB, instructional tuned SLMs significantly outperformed, with 2.802 vs 43.6 and 39.6.

% with mean MAE of ANX, DEP and CAL dropped from 1.401, 1.454 and 28.770 to 0.927, 0.715 and 7.571 respectively, and the mean accuracy of ACT rose from 19.838 to 21.8. On PMData, most tasks performance does not effectively improve from Few-shot and not even from Zero-shot for STRS, FATG and SQ. For best performance, the lowest MAE of READ and ANX from PMData and GLOBEM further decrease from 1.324 to 1.304 and 0.870 to 0.809, respectively; CAL from AW\_FB drops from 18.581 to 2.802 and ACT rises from 24.1 to 34.4. Compare to the best LLMs, SLMs are able to achieve superior performance than HealthAIpaca-lora-7b and even competitive performance than HealthAIpaca-lora-13b. For PMData, with 0.396 vs 0.34 and 0.53 in STRS, 1.304 vs 1.40 and 1.56 in READ. Similarly for FATG, SQ and other two datasets. For AW\_FB, instructional tuned SLMs significantly outperformed, with 2.802 vs 43.6 and 39.6.

% Across datasets, Phi-3-mini-4k and TinyLlama-1.1B delivered the most robust performance under LoRA. TinyLlama-1.1B attains the top FATG (63.2) with the lowest STRS (0.395), READ(1.304) and second best SQ(0.472), ANX(0.833). followed by Phi-3-mini-4k, which achieves the strongest ANX (0.809) and second best STRS (0.389), FATG (62.2), ACT (22.4). We further deploy them on iPhone 15 pro max to evaluate their real-time latency.

% In the few-shot setting, some models, including Qwen2-1.5B, Llama-3.2-1B, Llama-3.2-3B, and Phi-3.5-mini, tend to produce identical predictions on PMData tasks such as STRS and SQ, while some like SmolLM and TinyLlama failed to produce a valid answer. These behavior likely reflects their limited capacity to handle long and exemplar-heavy prompts, making them prone to collapse or to class-bias induced by the exemplars.

% Despite these advances, few-shot prompting showed limitations. Several models collapsed to identical predictions or produced invalid outputs, indicating difficulty with exemplar-heavy prompts. This highlights the need for adaptation strategies beyond prompting, including instruction-tuning or test-time adaptation.

% \begin{table*}[h]
% \centering
% \caption{SLMs performance across \textbf{PMData}, \textbf{LifeSnaps}, \textbf{GLOBEM}, and \textbf{AW-FB} under 4-bit quantization. Arrows show whether lower (↓) or higher (↑) is better. Best is in \textbf{bold}, second best is \underline{underlined}.}
% \label{tab:merged-datasets}
% \scriptsize
% \setlength{\tabcolsep}{6pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llcccccccccc}
% \toprule
% & & \multicolumn{4}{c}{\textbf{PMData}} & \multicolumn{2}{c}{\textbf{LifeSnaps}} & \multicolumn{2}{c}{\textbf{GLOBEM}} & \multicolumn{2}{c}{\textbf{AW-FB}} \\
% \cmidrule(lr){3-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
% & \textbf{Model} &
% \makecell{\textbf{STRS}\\(↓)} &
% \makecell{\textbf{READ}\\(↓)} &
% \makecell{\textbf{FATG}\\(↑)} &
% \makecell{\textbf{SQ}\\(↓)} &
% \makecell{\textbf{SR}\\(↓)} &
% \makecell{\textbf{SD}\\(↑)} &
% \makecell{\textbf{ANX}\\(↓)} &
% \makecell{\textbf{DEP}\\(↓)} &
% \makecell{\textbf{ACT}\\(↑)} &
% \makecell{\textbf{CAL}\\(↓)} \\
% \midrule
% \multirow{12}{*}{\makecell{\textbf{LLMs}\\(ZS)}}
% & MedAlpaca      & 0.76 ± 0.1 & 2.18 ± 0.1 & 46.8 ± 11 & 0.68 ± 0.0 & 1.17 ± 0.1 & 40.3 ± 1.6 & 1.23 ± 0.3 & \underline{0.89 ± 0.1} & 21.7 ± 4.4 & 35.0 ± 6.0 \\
% & PMC-Llama      & 1.33 ± 0.4 & 4.83 ± 1.2 & 0.00 ± 0.0 & 2.25 ± 0.0 & 1.21 ± 0.8 & 41.7 ± 8.3 & 2.33 ± 0.5 & 2.23 ± 0.3 & -          & 43.4 ± 1.2 \\
% & Asclepius      & 0.43 ± 0.0 & \textbf{1.44 ± 0.3} & 27.3 ± 10 & 0.45 ± 0.1 & -          & -          & \textbf{0.82 ± 0.2} & 1.10 ± 0.0 & -          & \textbf{28.9 ± 11} \\
% & ClinicalCamel  & 0.40 ± 0.1 & 2.11 ± 0.1 & 58.1 ± 3.2 & \textbf{0.37 ± 0.1} & 1.35 ± 0.1 & \underline{88.3 ± 1.6} & 0.97 ± 0.0 & 0.79 ± 0.1 & 16.3 ± 1.2 & 43.4 ± 5.3 \\
% & Flan-T5        & \textbf{0.36 ± 0.0} & 1.82 ± 0.1 & 56.8 ± 1.6 & 0.56 ± 0.0 & 2.20 ± 0.3 & 57.1 ± 3.5 & 2.84 ± 0.0 & 2.89 ± 0.0 & \underline{23.4 ± 0.0} & 66.0 ± 0.4 \\
% & Palmyra-Med    & 0.83 ± 0.1 & 5.01 ± 0.1 & 43.5 ± 15 & 0.44 ± 0.0 & \underline{1.03 ± 0.1} & 3.13 ± 0.2 & 2.07 ± 0.1 & 1.99 ± 0.2 & \textbf{29.7 ± 1.1} & 75.3 ± 5.5 \\
% & Llama 2        & 0.57 ± 0.2 & 2.86 ± 0.4 & 41.2 ± 13 & 0.89 ± 0.3 & -          & -          & 1.19 ± 0.1 & 1.23 ± 0.3 & -          & - \\
% & BioMedGPT      & \underline{0.37 ± 0.0} & 2.12 ± 0.2 & 61.2 ± 3.3 & \underline{0.41 ± 0.0} & \textbf{0.77 ± 0.2} & - & 0.95 ± 0.2 & \textbf{0.85 ± 0.1} & 12.2 ± 3.1 & - \\
% & BioMistral     & 0.55 ± 0.1 & 2.12 ± 0.2 & 56.6 ± 3.1 & 0.45 ± 0.0 & 1.59 ± 0.5 & \textbf{90.0 ± 0.0} & \underline{0.90 ± 0.1} & - & 18.4 ± 1.1 & 41.0 ± 4.3 \\
% & GPT-3.5        & -          & 2.38 ± 0.1 & \underline{70.8 ± 4.2} & 0.87 ± 0.0 & 1.21 ± 0.3 & 19.0 ± 10 & -          & -          & 13.8 ± 6.2 & 36.4 ± 0.0 \\
% & GPT-4          & -          & 2.22 ± 0.1 & \textbf{72.2 ± 2.0} & 0.73 ± 0.1 & 1.23 ± 0.1 & - & - & - & 22.6 ± 2.6 & 75.2 ± 8.2 \\
% & Gemini-Pro     & 0.79 ± 0.0 & \underline{1.69 ± 0.1} & 34.0 ± 9.8 & 0.78 ± 0.1 & 2.67 ± 1.1 & 84.6 ± 3.1 & 1.03 ± 0.1 & 0.95 ± 0.1 & 17.7 ± 0.0 & \underline{31.4 ± 1.9} \\
% \cmidrule{2-12}
% & Mean & 0.639 & 2.56 & 41.54 & 0.60 & 1.443 & 53.02 & 1.433 & 1.436 & 19.53 & 47.60 \\
% \midrule

% \multirow{4}{*}{\makecell{\textbf{LLMs}}}
% & HealthAlpaca-lora-7b  & 0.53 ± 0.0 & 1.40 ± 0.1 & 50.0 ± 13 & 0.58 ± 0.1 & 0.62 ± 0.1 & 61.7 ± 4.7 & 0.62 ± 0.0 & 0.51 ± 0.1 & 27.4 ± 5.0 & 43.6 ± 0.1 \\
% & HealthAlpaca-7b       & 0.31 ± 0.2 & 1.32 ± 0.2 & \textbf{70.7 ± 2.9} & 0.35 ± 0.1 & 0.62 ± 0.1 & 72.1 ± 8.9 & \textbf{0.46 ± 0.1} & 0.49 ± 0.2 & 41.7 ± 11 & 31.5 ± 6.4 \\
% & HealthAlpaca-lora-13b & 0.34 ± 0.0 & 1.56 ± 0.0 & 54.8 ± 9.7 & 0.39 ± 0.1 & 0.70 ± 0.0 & 92.0 ± 4.0 & 1.04 ± 0.1 & 0.67 ± 0.1 & 29.0 ± 0.0 & 39.6 ± 1.4 \\
% & HealthAlpaca-13b      & \textbf{0.21 ± 0.0} & \textbf{1.08 ± 0.2} & 61.2 ± 3.4 & \textbf{0.14 ± 0.0} & \textbf{0.32 ± 0.1} & \textbf{93.9 ± 3.1} & 0.95 ± 0.2 & \textbf{0.24 ± 0.0} & \textbf{51.0 ± 3.5} & \textbf{28.5 ± 5.6} \\
% \midrule
% \multirow{10}{*}{\makecell{\textbf{SLMs}\\(ZS)}}
% & gemma-2-2b-it   & 0.7174 & 2.0702 & 52.84 & 0.4716 & 1.5922 & -     & \underline{0.9097} & \textbf{0.5284} & -     & 105.12 \\
% & Phi-3-mini-4k   & 0.4548 & \textbf{1.5151} & 62.88 & 0.4816 & \underline{1.2803} & \textbf{80.00} & 1.0769 & 1.2642 & 17.39 & 93.80 \\
% & SmolLM-1.7B     & 1.4224 & 2.9900 & 11.04 & 1.0033 & -     & 44.44 & 2.5861 & 2.8744 & \textbf{21.74} & 277.21 \\
% & Qwen2-1.5B      & \textbf{0.3946} & 2.0268 & \underline{63.21} & \textbf{0.4515} & 2.2946 & 55.56 & 1.4174 & 1.6468 & 14.05 & 185.22 \\
% & TinyLlama-1.1B  & 0.4281 & 2.0569 & 51.17 & 0.4716 & -     & 44.44 & 2.3999 & 2.5775 & \underline{19.73} & 198.72 \\
% & Llama-3.2-1B    & \underline{0.3979} & \underline{1.8683} & \textbf{63.79} & 0.6889 & \textbf{1.2530} & 42.22 & 1.5066 & 1.8534 & 11.71 & 280.32 \\
% & Llama-3.2-3B    & 0.6689 & 2.2351 & 40.80 & 0.4649 & 1.6299 & 44.44 & 1.2642 & \underline{0.7542} & 15.72 & \textbf{19.70} \\
% & Phi-3.5-mini    & 0.4047 & 2.3386 & 61.20 & \underline{0.4548} & 1.4096 & \underline{73.33} & \textbf{0.8760} & 0.8428 & 15.38 & \underline{56.75} \\
% & Qwen2.5-1.5B    & 0.5552 & 2.2458 & 62.88 & 0.9264 & 2.1170 & 55.56 & 1.3645 & 1.6254 & 15.72 & 72.20 \\
% \cmidrule{2-12}
% & Mean            & 0.605  & 2.150  & 52.2  & 0.602  & 1.654  & 55.00 & 1.489 & 1.552 & 16.43 & 143.23 \\
% \midrule
% \multirow{10}{*}{\makecell{\textbf{SLMs}\\(FS-3)}}
% & gemma-2-2b-it   & 0.4816 & 1.6589 & 44.82 & 0.4883 & 1.653 & 53.3 & -     & -     & -     & - \\
% & Phi-3-mini-4k   & \underline{0.4114} & 1.6689 & 44.82 & \textbf{0.4515} & \textbf{0.574} & \underline{75.6} & \underline{0.880} & \textbf{0.535} & 19.4 & 54.983 \\
% & SmolLM-1.7B     & - & - & - & - & 0.740 & 53.3 & \textbf{0.870} & 0.582 & 15.4 & 18.972 \\
% & Qwen2-1.5B      & \underline{0.4114} & 1.6756 & \textbf{51.51} & \underline{0.4615} & \underline{0.661} & 57.8 & 0.883 & \textbf{0.535} & \underline{23.1} & 19.845 \\
% & TinyLlama-1.1B  & - & - & - & - & 0.820 & 44.4 & 2.933 & 3.043 & 14.4 & \textbf{17.902} \\
% & Llama-3.2-1B    & 0.4348 & 1.7324 & 49.83 & 0.5418 & 1.528 & 44.4 & 0.883 & \textbf{0.535} & 15.4 & \underline{18.472} \\
% & Llama-3.2-3B    & \underline{0.4114} & 1.7759 & \textbf{51.51} & 0.4682 & 1.014 & 42.2 & 1.194 & 1.117 & \textbf{24.1} & 19.270 \\
% & Phi-3.5-mini    & \underline{0.4114} & \textbf{1.4247} & \textbf{51.51} & \underline{0.4615} & 1.019 & \textbf{84.4} & 0.910 & \underline{0.548} & \textbf{24.1} & 32.941 \\
% & Qwen2.5-1.5B    & \textbf{0.3946} & \underline{1.4381} & \underline{37.12} & 0.7559 & 0.715 & 55.6 & 1.365 & 0.642 & 18.1 & \textbf{17.902} \\
% \cmidrule{2-12}
% & Mean            & 0.4224 & 1.6249 & 47.30 & 0.5184 & 0.969 & 56.8 & 1.240 & 0.942 & 19.2 & 25.036 \\
% \midrule
% % \multirow{10}{*}{\makecell{\textbf{SLMs}\\(lora-ID)}}
% % & gemma-2-2b-it   & - & - & - & 0.511 & \underline{0.723} & -     & 1.271 & 1.023 & \textbf{34.4} & \textbf{2.802} \\
% % & Phi-3-mini-4k   & \underline{0.398} & 2.144 & \underline{62.2} & 0.522 & 0.966 & \textbf{68.9} & \textbf{0.809} & 0.712 & \underline{22.4} & 9.673 \\
% % & SmolLM-1.7B     & 0.930 & 1.676 & 15.4 & 0.893 & 1.489 & 44.4 & 0.843 & \underline{0.539} & 16.1 & 18.868 \\
% % & Qwen2-1.5B      & 0.428 & 1.522 & \underline{62.2} & \underline{0.472} & 0.903 & 55.6 & 0.923 & 0.967 & 18.7 & 5.211 \\
% % & TinyLlama-1.1B  & \textbf{0.395} & \textbf{1.304} & \textbf{63.2} & \underline{0.472} & \textbf{0.667} & 55.6 & \underline{0.833} & 0.669 & 22.1 & 5.508 \\
% % & Llama-3.2-1B    & 0.428 & 2.251 & 49.8 & 0.809 & 1.090 & 48.9 & 0.860 & \textbf{0.535} & 19.2 & 5.775 \\
% % & Llama-3.2-3B    & 0.595 & 1.532 & 40.8 & \textbf{0.465} & 0.858 & 53.3 & 0.883 & \textbf{0.535} & 22.1 & \underline{3.640} \\
% % & Phi-3.5-mini    & 0.485 & 1.548 & \underline{62.2} & 0.920 & 0.981 & \underline{62.2} & 0.880 & 0.659 & 19.4 & 12.091 \\
% % & Qwen2.5-1.5B    & 0.866 & \underline{1.485} & 13.0 & 0.866 & 1.891 & 55.6 & 1.037 & 0.793 & 21.7 & 4.569 \\
% % & Mean            & 0.566 & 1.683 & 46.1 & 0.659 & 1.063 & 55.6 & 0.927 & 0.715 & 21.8 & 7.571 \\
% % \midrule
% % \multirow{10}{*}{\makecell{\textbf{SLMs}\\(FT-ID)}}
% % & gemma-2-2b-it   & \textbf{0.351} & \textbf{1.304} & 62.9 & \textbf{0.452} & 0.625 & 55.6 & 0.883 & \underline{0.535} & \underline{53.2} & \underline{2.147} \\
% % & Phi-3-mini-4k   & 0.398 & 1.535 & 62.9 & 0.468 & \underline{0.549} & \textbf{86.7} & \textbf{0.803} & 0.542 & 19.4 & 28.194 \\
% % & SmolLM-1.7B     & 0.732 & 2.993 & 18.1 & 1.672 & 14.757 & 43.2 & 1.997 & 0.686 & 16.0 & - \\
% % & Qwen2-1.5B      & 0.395 & \textbf{1.304} & \underline{63.2} & 0.478 & 0.820 & 55.6 & 1.050 & \underline{0.535} & 38.1 & 3.846 \\
% % & TinyLlama-1.1B  & 0.398 & \underline{1.331} & \underline{63.2} & \underline{0.455} & 0.675 & 44.4 & \underline{0.863} & \underline{0.535} & 38.1 & 2.312 \\
% % & Llama-3.2-1B    & 0.395 & 2.160 & \textbf{64.5} & 0.462 & 0.681 & 55.6 & - & - & 38.5 & 2.050 \\
% % & Llama-3.2-3B    & \underline{0.385} & \textbf{1.304} & 56.9 & \textbf{0.452} & 0.574 & - & 0.873 & \textbf{0.532} & \textbf{55.4} & \textbf{1.712} \\
% % & Phi-3.5-mini    & 0.535 & 1.512 & 61.2 & 0.508 & \textbf{0.450} & \underline{80.0} & 0.886 & 0.549 & 16.4 & 6.187 \\
% % & Qwen2.5-1.5B    & 0.682 & 1.446 & 39.6 & \underline{0.455} & 1.394 & 71.1 & 0.953 & 0.695 & 15.4 & 5.790 \\
% % & Mean            & 0.474 & 1.655 & 54.7 & 0.600 & 2.281 & 61.5 & 1.038 & 0.576 & 32.3 & 6.530 \\
% % \midrule

% % \midrule 

% %ID
% \multirow{10}{*}{\makecell{\textbf{SLMs}\\(lora)}}
% & gemma-2-2b-it        & -      & -      & -    & 0.511 & \underline{0.723} & -     & 1.271 & 1.023 & \textbf{34.4} & \textbf{2.802} \\
% & Phi-3-mini-4k        & \underline{0.398} & 2.144 & \underline{62.2} & 0.522 & 0.966 & \textbf{68.9} & \textbf{0.809} & 0.712 & \underline{22.4} & 9.673 \\
% & SmolLM-1.7B          & 0.930  & 1.676  & 15.4 & 0.893 & 1.489 & 44.4  & 0.843 & \underline{0.539} & 16.1 & 18.868 \\
% & Qwen2-1.5B           & 0.428  & 1.522  & \underline{62.2} & \underline{0.472} & 0.903 & 55.6  & 0.923 & 0.967 & 18.7 & 5.211 \\
% & TinyLlama-1.1B       & \textbf{0.395} & \textbf{1.304} & \textbf{63.2} & \underline{0.472} & \textbf{0.667} & 55.6  & \underline{0.833} & 0.669 & 22.1 & 5.508 \\
% & Llama-3.2-1B         & 0.428  & 2.251  & 49.8 & 0.809 & 1.090 & 48.9  & 0.860 & \textbf{0.535} & 19.2 & 5.775 \\
% & Llama-3.2-3B         & 0.595  & 1.532  & 40.8 & \textbf{0.465} & 0.858 & 53.3  & 0.883 & \textbf{0.535} & 22.1 & \underline{3.640} \\
% & Phi-3.5-mini         & 0.485  & 1.548  & \underline{62.2} & 0.920 & 0.981 & \underline{62.2} & 0.880 & 0.659 & 19.4 & 12.091 \\
% & Qwen2.5-1.5B         & 0.866  & \underline{1.485} & 13.0 & 0.866 & 1.891 & 55.6  & 1.037 & 0.793 & 21.7 & 4.569 \\
% \cmidrule{2-12}
% & Mean                 & 0.566  & 1.683  & 46.1 & 0.659 & 1.063 & 55.6  & 0.927 & 0.715 & 21.8 & 7.571 \\
% \midrule

% \multirow{10}{*}{\makecell{\textbf{SLMs}\\(FT)}}
% & gemma-2-2b-it        & \textbf{0.351} & \textbf{1.304} & 62.9 & \textbf{0.452} & 0.625 & 55.6 & 0.883 & \underline{0.535} & \underline{53.2} & \underline{2.147} \\
% & Phi-3-mini-4k        & 0.398 & 1.535 & 62.9 & 0.468 & \underline{0.549} & \textbf{86.7} & \textbf{0.803} & 0.542 & 19.4 & 28.194 \\
% & SmolLM-1.7B          & 0.732 & 2.993 & 18.1 & 1.672 & 14.757 & 43.2 & 1.997 & 0.686 & 16.0 & - \\
% & Qwen2-1.5B           & 0.395 & \textbf{1.304} & \underline{63.2} & 0.478 & 0.820 & 55.6 & 1.050 & \underline{0.535} & 38.1 & 3.846 \\
% & TinyLlama-1.1B       & 0.398 & \underline{1.331} & \underline{63.2} & \underline{0.455} & 0.675 & 44.4 & \underline{0.863} & \underline{0.535} & 38.1 & 2.312 \\
% & Llama-3.2-1B         & 0.395 & 2.160 & \textbf{64.5} & 0.462 & 0.681 & 55.6 & - & - & 38.5 & 2.050 \\
% & Llama-3.2-3B         & \underline{0.385} & \textbf{1.304} & 56.9 & \textbf{0.452} & 0.574 & - & 0.873 & \textbf{0.532} & \textbf{55.4} & \textbf{1.712} \\
% & Phi-3.5-mini         & 0.535 & 1.512 & 61.2 & 0.508 & \textbf{0.450} & \underline{80.0} & 0.886 & 0.549 & 16.4 & 6.187 \\
% & Qwen2.5-1.5B         & 0.682 & 1.446 & 39.6 & \underline{0.455} & 1.394 & 71.1 & 0.953 & 0.695 & 15.4 & 5.790 \\
% \cmidrule{2-12}
% & Mean                 & 0.474 & 1.655 & 54.7 & 0.600 & 2.281 & 61.5 & 1.038 & 0.576 & 32.3 & 6.530 \\



% %MD

% % \multirow{10}{*}{\makecell{\textbf{SLMs}\\(lora)}}
% % & gemma-2-2b-it   & - & - & - & - & 1.403 & \underline{55.6} & \underline{0.786} & \textbf{0.525} & 16.05 & \underline{4.205} \\
% % & Phi-3-mini-4k   & \underline{0.405} & 2.709 & 58.7 & 0.689 & \underline{0.999} & \underline{55.6} & 0.901 & 1.213 & 19.59 & 13.298 \\
% % & SmolLM-1.7B     & 0.806 & 1.823 & 5.4 & 1.037 & 2.034 & 44.4 & 2.656 & 3.124 & \underline{21.07} & - \\
% % & Qwen2-1.5B      & \textbf{0.395} & \textbf{1.304} & \textbf{63.2} & \underline{0.469} & 1.188 & 44.4 & 1.050 & 0.769 & 15.05 & \textbf{3.426} \\
% % & TinyLlama-1.1B  & 0.582 & \underline{1.535} & 48.8 & \textbf{0.468} & 0.748 & 44.4 & \textbf{0.780} & 0.592 & 15.72 & 6.272 \\
% % & Llama-3.2-1B    & 1.047 & 4.226 & \underline{60.5} & 0.503 & \textbf{0.676} & \underline{55.6} & 0.883 & 0.565 & 17.06 & 8.384 \\
% % & Llama-3.2-3B    & 0.435 & - & 36.5 & - & - & - & 0.843 & \underline{0.545} & - & - \\
% % & Phi-3.5-mini    & 0.428 & 1.559 & 40.0 & 0.679 & 0.730 & \textbf{66.7} & 0.896 & 0.920 & 20.40 & 13.687 \\
% % & Qwen2.5-1.5B    & 0.514 & 2.341 & - & - & 1.570 & 40.0 & 1.041 & 0.589 & \textbf{23.38} & 4.576 \\
% % \cmidrule{2-12}
% % & Mean            & 0.576 & 2.097 & 44.3 & 0.578 & 1.061 & 50.6 & 1.092 & 0.872 & 18.54 & 7.978 \\
% % \midrule
% % \multirow{10}{*}{\makecell{\textbf{SLMs}\\(FT)}}
% % & gemma-2-2b-it   & \underline{0.361} & \underline{1.304} & \textbf{63.9} & \underline{0.434} & \textbf{0.404} & 71.1 & 0.883 & \textbf{0.535} & \textbf{53.20} & \textbf{2.145} \\
% % & Phi-3-mini-4k   & 0.428 & 1.492 & 62.9 & 0.475 & 0.868 & \textbf{91.1} & \textbf{0.826} & 0.622 & 20.10 & 38.563 \\
% % & SmolLM-1.7B     & 0.769 & 3.321 & 12.0 & 1.141 & 9.500 & 44.2 & 2.181 & 2.605 & 16.10 & 788.494 \\
% % & Qwen2-1.5B      & \textbf{0.395} & \textbf{1.291} & 63.2 & 0.482 & 0.922 & 55.6 & 1.054 & 0.769 & 17.40 & 4.847 \\
% % & TinyLlama-1.1B  & 0.696 & 1.926 & 48.1 & 0.448 & 0.684 & 44.4 & 0.883 & \underline{0.542} & 12.40 & \underline{2.640} \\
% % & Llama-3.2-1B    & 0.585 & 1.358 & 36.5 & 0.468 & \underline{0.678} & 44.4 & \underline{0.877} & \underline{0.542} & 36.50 & 2.863 \\
% % & Llama-3.2-3B    & 0.451 & 1.312 & \textbf{63.9} & 0.455 & - & - & 0.883 & 0.535 & \underline{46.90} & 2.805 \\
% % & Phi-3.5-mini    & 0.441 & 1.659 & 60.2 & 0.441 & - & \underline{77.8} & 0.833 & 0.692 & 22.00 & 19.703 \\
% % & Qwen2.5-1.5B    & 0.395 & 1.762 & \underline{63.4} & \textbf{0.428} & 1.790 & 55.6 & 1.043 & 0.769 & 14.70 & 7.690 \\
% % \cmidrule{2-12}
% % & Mean            & 0.497 & 1.638 & 52.7 & 0.586 & 1.510 & 61.2 & 1.186 & 0.850 & 26.70 & 96.870 \\


% \bottomrule
% \end{tabular}
% }
% \end{table*}

% \end{document}

% \begin{table*}[ht!]
% \centering
% \caption{Comparison of Model Performance on LifeSnaps, GLOBEM, and AW\_FB after multi-dataset Instructional Fine-tuning. Arrows indicate whether lower (↓) or higher (↑) values are better. The best result is \textbf{bolded} and the second best result is \underline{underlined}. ID refers to Individual-dataset Finetuning, while MD refers to Multi-dataset Finetuning}
% \label{tab:finetuned_taskgroup_off on pmdata - Multi-dataset}
% \scriptsize
% \begin{tabular}{llcccc}
% \toprule
% & \textbf{Model} & \textbf{STRS (↓)} & \textbf{READ (↓)} & \textbf{FATG (↑)} & \textbf{SQ (↓)} \\
% \midrule
% \multirow{4}{*}{\centering\arraybackslash\begin{tabular}[c]{@{}c@{}}\textbf{LLMs}\\\end{tabular}} 
% & HealthAlpaca-lora-7b   & 0.53 ± 0.0 & 1.40 ± 0.1 & 50.0 ± 13 & 0.58 ± 0.1 \\
% & HealthAlpaca-7b        & 0.31 ± 0.2 & 1.32 ± 0.2 & \textbf{70.7 ± 2.9} & 0.35 ± 0.1 \\
% & HealthAlpaca-lora-13b  & 0.34 ± 0.0 & 1.56 ± 0.0 & 54.8 ± 9.7 & 0.39 ± 0.1 \\
% & HealthAlpaca-13b       & \textbf{0.21 ± 0.0} & \textbf{1.08 ± 0.2} & 61.2 ± 3.4 & \textbf{0.14 ± 0.0} \\

% \midrule
% \multirow{9}{*}{\centering\arraybackslash\begin{tabular}[c]{@{}c@{}}\textbf{SLMs}\\(ZS)\end{tabular}}
% & gemma-2-2b-it & 0.7174 & 2.0702 & 52.84 & 0.4716 \\
% & Phi-3-mini-4k & 0.4548 & \textbf{1.5151} & 62.88 & 0.4816 \\
% & SmolLM-1.7B & 1.4224 & 2.9900 & 11.04 & 1.0033 \\
% & Qwen2-1.5B & \textbf{0.3946} & 2.0268 & \underline{63.21} & \textbf{0.4515} \\
% & TinyLlama-1.1B & 0.4281 & 2.0569 & 51.17 & 0.4716 \\
% & Llama-3.2-1B & \underline{0.3979} & \underline{1.8683} & \textbf{63.79} & 0.6889 \\
% & Llama-3.2-3B & 0.6689 & 2.2351 & 40.80 & 0.4649 \\
% & Phi-3.5-mini & 0.4047 & 2.3386 & 61.20 & \underline{0.4548} \\
% & Qwen2.5-1.5B & 0.5552 & 2.2458 & 62.88 & 0.9264 \\
% \cmidrule{2-6}
% & Mean & 0.605 & 2.150 & 52.2 & 0.602 \\

% \midrule
% \multirow{9}{*}{\centering\arraybackslash\begin{tabular}[c]{@{}c@{}}\textbf{SLMs}\\(FS-3)\end{tabular}}
% & gemma-2-2b-it             & 0.4816              & 1.6589              & 44.82              & 0.4883 \\
% & Phi-3-mini-4k             & \underline{0.4114}  & 1.6689              & 44.82              & \textbf{0.4515} \\
% & SmolLM-1.7B            & -                   & -                   & -                   & - \\
% & Qwen2-1.5B             & \underline{0.4114}  & 1.6756              & \textbf{51.51}     & \underline{0.4615} \\
% & TinyLlama-1.1B         & -                   & -                   & -                   & - \\
% & Llama-3.2-1B           & 0.4348              & 1.7324              & 49.83              & 0.5418 \\
% & Llama-3.2-3B           & \underline{0.4114}  & 1.7759              & \textbf{51.51}     & 0.4682 \\
% & Phi-3.5-mini           & \underline{0.4114}  & \textbf{1.4247}     & \textbf{51.51}     & \underline{0.4615} \\
% & Qwen2.5-1.5B           & \textbf{0.3946}     & \underline{1.4381}  & \underline{37.12}  & 0.7559 \\
% \cmidrule{2-6}
% & Mean                   & 0.4224 & 1.6249 & 47.30 & 0.5184 \\

% \midrule
% \multirow{9}{*}{\centering\arraybackslash\begin{tabular}[c]{@{}c@{}}\textbf{SLMs}\\(lora-ID)\end{tabular}} 
% & gemma-2-2b-it        & -             & -             & - & 0.511 \\
% & Phi-3-mini-4k        & \underline{0.398} & 2.144 & \underline{62.2} & 0.522 \\
% & SmolLM-1.7B       & 0.930         & 1.676         & 15.4 & 0.893 \\
% & Qwen2-1.5B        & 0.428         & 1.522         & \underline{62.2} & \underline{0.472} \\
% & TinyLlama-1.1B    & \textbf{0.395} & \textbf{1.304} & \textbf{63.2} & \underline{0.472} \\
% & Llama-3.2-1B      & 0.428         & 2.251         & 49.8 & 0.809 \\
% & Llama-3.2-3B      & 0.595         & 1.532         & 40.8 & \textbf{0.465} \\
% & Phi-3.5-mini      & 0.485         & 1.548         & \underline{62.2} & 0.920 \\
% & Qwen2.5-1.5B      & 0.866         & \underline{1.485} & 13.0 & 0.866 \\
% \cmidrule{2-6}
% & Mean              & 0.566 & 1.683 & 46.1 & 0.659 \\

% \midrule
% \multirow{9}{*}{\centering\arraybackslash\begin{tabular}[c]{@{}c@{}}\textbf{SLMs}\\(FT-ID)\end{tabular}} 
% & gemma-2-2b-it        & \textbf{0.351} & \textbf{1.304} & 62.9 & \textbf{0.452} \\
% & Phi-3-mini-4k        & 0.398 & 1.535 & 62.9 & 0.468 \\
% & SmolLM-1.7B       & 0.732 & 2.993 & 18.1 & 1.672 \\
% & Qwen2-1.5B        & 0.395 & \textbf{1.304} & \underline{63.2} & 0.478 \\
% & TinyLlama-1.1B    & 0.398 & \underline{1.331} & \underline{63.2} & \underline{0.455} \\
% & Llama-3.2-1B      & 0.395 & 2.160 & \textbf{64.5} & 0.462 \\
% & Llama-3.2-3B      & \underline{0.385} & \textbf{1.304} & 56.9 & \textbf{0.452} \\
% & Phi-3.5-mini      & 0.535 & 1.512 & 61.2 & 0.508 \\
% & Qwen2.5-1.5B      & 0.682 & 1.446 & 39.6 & \underline{0.455} \\
% \cmidrule{2-6}
% & Mean              & 0.474 & 1.655 & 54.7 & 0.600 \\

% \midrule
% \multirow{9}{*}{\centering\arraybackslash\begin{tabular}[c]{@{}c@{}}\textbf{SLMs}\\(lora)\end{tabular}} 
% & gemma-2-2b-it        & -             & - & - & - \\
% & Phi-3-mini-4k     & \underline{0.405} & 2.709 & 58.7 & 0.689 \\
% & SmolLM-1.7B       & 0.806         & 1.823 & 5.4  & 1.037 \\
% & Qwen2-1.5B        & \textbf{0.395} & \textbf{1.304} & \textbf{63.2} & \underline{0.469} \\
% & TinyLlama-1.1B    & 0.582       & \underline{1.535} & 48.8 & \textbf{0.468} \\
% & Llama-3.2-1B      & 1.047         & 4.226 & \underline{60.5} & 0.503 \\
% & Llama-3.2-3B      & 0.435         & - & 36.5 & - \\
% & Phi-3.5-mini      & 0.428         & 1.559 & 40.0 & 0.679 \\
% & Qwen2.5-1.5B      & 0.514         & 2.341 & - & - \\
% \cmidrule{2-6}
% & Mean              & 0.576 & 2.097 & 44.3 & 0.578 \\

% \midrule
% \multirow{9}{*}{\centering\arraybackslash\begin{tabular}[c]{@{}c@{}}\textbf{SLMs}\\(FT)\end{tabular}} 
% & gemma-2-2b-it             & \underline{0.361} & \underline{1.304} & \textbf{63.9} & \underline{0.434} \\
% & Phi-3-mini-4k          & 0.428 & 1.492 & 62.9 & 0.475 \\
% & SmolLM-1.7B            & 0.769 & 3.321 & 12.0 & 1.141 \\
% & Qwen2-1.5B             & \textbf{0.395} & \textbf{1.291} & 63.2 & 0.482 \\
% & TinyLlama-1.1B         & 0.696 & 1.926 & 48.1 & 0.448 \\
% & Llama-3.2-1B           & 0.585 & 1.358 & 36.5 & 0.468 \\
% & Llama-3.2-3B           & 0.451 & 1.312 & \textbf{63.9} & 0.455 \\
% & Phi-3.5-mini           & 0.441 & 1.659 & 60.2 & 0.441 \\
% & Qwen2.5-1.5B           & 0.395 & 1.762 & \underline{63.4} & \textbf{0.428} \\
% \cmidrule{2-6}
% & Mean                   & 0.497 & 1.638 & 52.7 & 0.586 \\

% \bottomrule
% \end{tabular}%
% \end{table*}


% \begin{table*}[h!]
% \centering
% \caption{Comparison of Model Performance on LifeSnaps, GLOBEM, and AW\_FB after Multi-dataset Instructional Fine-tuning. Arrows indicate whether lower (↓) or higher (↑) values are better. The Best results are shown in \textbf{bold} and the second best results are \underline{underlined}. ID refers to Individual-dataset Finetuning, while MD refers to Multi-dataset Finetuning}
% \label{tab:finetuned_taskgroup_off on lifesnaps, globem and aw_fb - Multi-dataset}
% \resizebox{1\columnwidth}{!}{
% \begin{tabular}{llcccccc}
% \toprule
% & \textbf{Model} & \textbf{SR (↓)} & \textbf{SD (↑)} & \textbf{ANX (↓)} & \textbf{DEP (↓)} & \textbf{ACT (↑)} & \textbf{CAL (↓)} \\
% \midrule
% \multirow{4}{*}{\centering\arraybackslash\begin{tabular}[c]{@{}c@{}}\textbf{LLMs}\\\end{tabular}} 
% & HealthAlpaca-lora-7b   & 0.62 ± 0.1 & 61.7 ± 4.7 & 0.62 ± 0.0 & 0.51 ± 0.1 & 27.4 ± 5.0 & 43.6 ± 0.1 \\
% & HealthAlpaca-7b        & 0.62 ± 0.1 & 72.1 ± 8.9 & \textbf{0.46 ± 0.1} & 0.49 ± 0.2 & 41.7 ± 11 & 31.5 ± 6.4 \\
% & HealthAlpaca-lora-13b  & 0.70 ± 0.0 & 92.0 ± 4.0 & 1.04 ± 0.1 & 0.67 ± 0.1 & 29.0 ± 0.0 & 39.6 ± 1.4 \\
% & HealthAlpaca-13b       & \textbf{0.32 ± 0.1} & \textbf{93.9 ± 3.1} & 0.95 ± 0.2 & \textbf{0.24 ± 0.0} & \textbf{51.0 ± 3.5} & \textbf{28.5 ± 5.6} \\

% \midrule
% \multirow{9}{*}{\centering\arraybackslash\begin{tabular}[c]{@{}c@{}}\textbf{SLMs}\\(ZS)\end{tabular}} 
% & gemma-2-2b-it      & 1.5922  & - & \underline{0.9097} & \textbf{0.5284} & - & 105.12 \\
% & Phi-3-mini-4k      & \underline{1.2803}  & \textbf{80.00} & 1.0769 & 1.2642 & 17.39 & 93.80  \\
% & SmolLM-1.7B     & -  & 44.44 & 2.5861 & 2.8744 & \textbf{21.74} & 277.21 \\
% & Qwen2-1.5B      & 2.2946  & 55.56 & 1.4174 & 1.6468 & 14.05 & 185.22 \\
% & TinyLlama-1.1B  & - & 44.44 & 2.3999 & 2.5775 & \underline{19.73} & 198.72 \\
% & Llama-3.2-1B    & \textbf{1.2530} & 42.22 & 1.5066 & 1.8534 & 11.71 & 280.32 \\
% & Llama-3.2-3B    & 1.6299  & 44.44 & 1.2642 & \underline{0.7542} & 15.72 & \textbf{19.70} \\
% & Phi-3.5-mini    & 1.4096  & \underline{73.33} & \textbf{0.8760} & 0.8428 & 15.38 & \underline{56.75}  \\
% & Qwen2.5-1.5B    & 2.1170  & 55.56 & 1.3645 & 1.6254 & 15.72 & 72.20  \\
% \cmidrule{2-8}
% & Mean & 1.654 & 55.00 & 1.489 & 1.552 & 16.43 & 143.23 \\


% \midrule
% \multirow{9}{*}{\centering\arraybackslash\begin{tabular}[c]{@{}c@{}}\textbf{SLMs}\\(FS-3)\end{tabular}} 
% & gemma-2-2b-it             & 1.653 & 53.3 & -     & -     & -     & - \\
% & Phi-3-mini-4k             & \textbf{0.574} & \underline{75.6} & \underline{0.880} & \textbf{0.535} & 19.4 & 54.983 \\
% & SmolLM-1.7B            & 0.740 & 53.3 & \textbf{0.870} & 0.582 & 15.4 & 18.972 \\
% & Qwen2-1.5B             & \underline{0.661} & 57.8 & 0.883 & \textbf{0.535} & \underline{23.1} & 19.845 \\
% & TinyLlama-1.1B         & 0.820 & 44.4 & 2.933 & 3.043 & 14.4 & \textbf{17.902} \\
% & Llama-3.2-1B           & 1.528 & 44.4 & 0.883 & \textbf{0.535} & 15.4 & \underline{18.472} \\
% & Llama-3.2-3B           & 1.014 & 42.2 & 1.194 & 1.117 & \textbf{24.1} & 19.270 \\
% & Phi-3.5-mini           & 1.019 & \textbf{84.4} & 0.910 & \underline{0.548} & \textbf{24.1} & 32.941 \\
% & Qwen2.5-1.5B           & 0.715 & 55.6 & 1.365 & 0.642 & 18.1 & \textbf{17.902} \\
% \cmidrule{2-8}
% & Mean                  & 0.969 & 56.8 & 1.240 & 0.942 & 19.2 & 25.036 \\

% \midrule
% \multirow{9}{*}{\centering\arraybackslash\begin{tabular}[c]{@{}c@{}}\textbf{SLMs} \\ (lora-ID)\end{tabular}} 
% & gemma-2-2b-it        & \underline{0.723} & -     & 1.271 & 1.023 & \textbf{34.4} & \textbf{2.802} \\
% & Phi-3-mini-4k     & 0.966 & \textbf{68.9} & \textbf{0.809} & 0.712 & \underline{22.4} & 9.673 \\
% & SmolLM-1.7B       & 1.489 & 44.4 & 0.843 & \underline{0.539} & 16.1 & 18.868 \\
% & Qwen2-1.5B        & 0.903 & 55.6 & 0.923 & 0.967 & 18.7 & 5.211 \\
% & TinyLlama-1.1B    & \textbf{0.667} & 55.6 & \underline{0.833} & 0.669 & 22.1 & 5.508 \\
% & Llama-3.2-1B      & 1.090 & 48.9 & 0.860 & \textbf{0.535} & 19.2 & 5.775 \\
% & Llama-3.2-3B      & 0.858 & 53.3 & 0.883 & \textbf{0.535} & 22.1 & \underline{3.640} \\
% & Phi-3.5-mini      & 0.981 & \underline{62.2} & 0.880 & 0.659 & 19.4 & 12.091 \\
% & Qwen2.5-1.5B      & 1.891 & 55.6 & 1.037 & 0.793 & 21.7 & 4.569 \\
% \cmidrule{2-8}
% & Mean              & 1.063 & 55.6  & 0.927 & 0.715 & 21.8 & 7.571 \\

% \midrule
% \multirow{9}{*}{\centering\arraybackslash\begin{tabular}[c]{@{}c@{}}\textbf{SLMs} \\(FT-ID)\end{tabular}} 
% & gemma-2-2b-it        & 0.625 & 55.6 & 0.883 & \underline{0.535} & \underline{53.2} & \underline{2.147} \\
% & Phi-3-mini-4k     & \underline{0.549} & \textbf{86.7} & \textbf{0.803} & 0.542 & 19.4 & 28.194 \\
% & SmolLM-1.7B       & 14.757 & 43.2 & 1.997 & 0.686 & 16.0 & - \\
% & Qwen2-1.5B        & 0.820 & 55.6 & 1.050 & \underline{0.535} & 38.1 & 3.846 \\
% & TinyLlama-1.1B    & 0.675 & 44.4 & \underline{0.863} & \underline{0.535} & 38.1 & 2.312 \\
% & Llama-3.2-1B      & 0.681 & 55.6 & - & - & 38.5 & 2.050 \\
% & Llama-3.2-3B      & 0.574 & - & 0.873 & \textbf{0.532} & \textbf{55.4} & \textbf{1.712} \\
% & Phi-3.5-mini      & \textbf{0.450} & \underline{80.0} & 0.886 & 0.549 & 16.4 & 6.187 \\
% & Qwen2.5-1.5B      & 1.394 & 71.1 & 0.953 & 0.695 & 15.4 & 5.790 \\
% \cmidrule{2-8}
% & Mean              & 2.281 & 61.5 & 1.038 & 0.576 & 32.3 & 6.530 \\

% \midrule
% \multirow{9}{*}{\centering\arraybackslash\begin{tabular}[c]{@{}c@{}}\textbf{SLMs} \\ (lora)\end{tabular}} 
% & gemma-2-2b-it        & 1.403 & \underline{55.6} & \underline{0.786} & \textbf{0.525} & 16.05 & \underline{4.205} \\
% & Phi-3-mini-4k        & \underline{0.999} & \underline{55.6} & 0.901 & 1.213 & 19.59 & 13.298 \\
% & SmolLM-1.7B          & 2.034 & 44.4 & 2.656 & 3.124 & \underline{21.07} & - \\
% & Qwen2-1.5B           & 1.188 & 44.4 & 1.050 & 0.769 & 15.05 & \textbf{3.426} \\
% & TinyLlama-1.1B       & 0.748 & 44.4 & \textbf{0.780} & 0.592 & 15.72 & 6.272 \\
% & Llama-3.2-1B         & \textbf{0.676} & \underline{55.6} & 0.883 & 0.565 & 17.06 & 8.384 \\
% & Llama-3.2-3B         & - & - & 0.843 & \underline{0.545} & - & - \\
% & Phi-3.5-mini         & 0.730 & \textbf{66.7} & 0.896 & 0.920 & 20.40 & 13.687 \\
% & Qwen2.5-1.5B         & 1.570 & 40.0 & 1.041 & 0.589 & \textbf{23.38} & 4.576 \\
% \cmidrule{2-8}
% & Mean                 & 1.061 & 50.6 & 1.092 & 0.872 & 18.54 & 7.978 \\

% \midrule
% \multirow{9}{*}{\centering\arraybackslash\begin{tabular}[c]{@{}c@{}}\textbf{SLMs} \\(FT)\end{tabular}} 
% & gemma-2-2b-it             & \textbf{0.404} & 71.1 & 0.883 & \textbf{0.535} & \textbf{53.20} & \textbf{2.145} \\
% & Phi-3-mini-4k          & 0.868 & \textbf{91.1} & \textbf{0.826} & 0.622 & 20.10 & 38.563 \\
% & SmolLM-1.7B            & 9.500 & 44.2 & 2.181 & 2.605 & 16.10 & 788.494 \\
% & Qwen2-1.5B             & 0.922 & 55.6 & 1.054 & 0.769 & 17.40 & 4.847 \\
% & TinyLlama-1.1B    & 0.684 & 44.4 & 0.883 & \underline{0.542} & 12.40 & \underline{2.640} \\
% & Llama-3.2-1B           & \underline{0.678} & 44.4 & \underline{0.877} & \underline{0.542} & 36.50 & 2.863 \\
% & Llama-3.2-3B           & - & - & 0.883 & 0.535 & \underline{46.90} & 2.805 \\
% & Phi-3.5-mini           & - & \underline{77.8} & 0.833 & 0.692 & 22.00 & 19.703 \\
% & Qwen2.5-1.5B           & 1.790 & 55.6 & 1.043 & 0.769 & 14.70 & 7.690 \\
% \cmidrule{2-8}
% & Mean                   & 1.510 & 61.2 & 1.186 & 0.850 & 26.70 & 96.870 \\

% \bottomrule
% \end{tabular} }
% \end{table*}




% \begin{table*}[h]
% \centering
% \caption{Performance of SLMs under \textbf{zero-shot}, \textbf{Few-shot}, and \textbf{LoRA} settings across \textbf{PMData}, \textbf{LifeSnaps}, \textbf{GLOBEM}, and \textbf{AW-FB}, evaluated with 4-bit quantization.}
% \label{tab:others}
% \scriptsize
% \setlength{\tabcolsep}{6pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llcccccccccc}
% \toprule
% & & \multicolumn{4}{c}{\textbf{PMData}} & \multicolumn{2}{c}{\textbf{LifeSnaps}} & \multicolumn{2}{c}{\textbf{GLOBEM}} & \multicolumn{2}{c}{\textbf{AW-FB}} \\
% \cmidrule(lr){3-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
% & \textbf{Model} &
% \makecell{\textbf{STRS}\\(↓)} &
% \makecell{\textbf{READ}\\(↓)} &
% \makecell{\textbf{FATG}\\(↑)} &
% \makecell{\textbf{SQ}\\(↓)} &
% \makecell{\textbf{SR}\\(↓)} &
% \makecell{\textbf{SD}\\(↑)} &
% \makecell{\textbf{ANX}\\(↓)} &
% \makecell{\textbf{DEP}\\(↓)} &
% \makecell{\textbf{ACT}\\(↑)} &
% \makecell{\textbf{CAL}\\(↓)} \\
% \midrule
% \multirow{2}{*}{\makecell{\textbf{LLMs}\\(lora)}} 
% & HealthAlpaca-lora-7b  & 0.53 ± 0.0 & \textbf{1.40 ± 0.1} & 50.0 ± 13 & 0.58 ± 0.1 & 0.62 ± 0.1 & 61.7 ± 4.7 & \textbf{0.62 ± 0.0} & 0.51 ± 0.1 & 27.4 ± 5.0 & 43.6 ± 0.1 \\
% % & HealthAlpaca-7b       & 0.31 ± 0.2 & 1.32 ± 0.2 & \textbf{70.7 ± 2.9} & 0.35 ± 0.1 & 0.62 ± 0.1 & 72.1 ± 8.9 & \textbf{0.46 ± 0.1} & 0.49 ± 0.2 & 41.7 ± 11 & 31.5 ± 6.4 \\
% & HealthAlpaca-lora-13b & \textbf{0.34 ± 0.0} & 1.56 ± 0.0 & \textbf{54.8 ± 9.7} & \textbf{0.39 ± 0.1} & \textbf{0.70 ± 0.0} & \textbf{92.0 ± 4.0} & 1.04 ± 0.1 & \textbf{0.67 ± 0.1} & \textbf{29.0 ± 0.0} & \textbf{39.6 ± 1.4} \\
% % & HealthAlpaca-13b      & \textbf{0.21 ± 0.0} & \textbf{1.08 ± 0.2} & 61.2 ± 3.4 & \textbf{0.14 ± 0.0} & \textbf{0.32 ± 0.1} & \textbf{93.9 ± 3.1} & 0.95 ± 0.2 & \textbf{0.24 ± 0.0} & \textbf{51.0 ± 3.5} & \textbf{28.5 ± 5.6} \\
% \midrule

% \multirow{10}{*}{\makecell{\textbf{SLMs}\\(ZS)}}
% & gemma-2-2b-it   & 0.7174 & 2.0702 & 52.84 & 0.4716 & 1.5922 & -     & \underline{0.9097} & \textbf{0.5284} & -     & 105.12 \\
% & Phi-3-mini-4k   & 0.4548 & \textbf{1.5151} & 62.88 & 0.4816 & \underline{1.2803} & \textbf{80.00} & 1.0769 & 1.2642 & 17.39 & 93.80 \\
% & SmolLM-1.7B     & 1.4224 & 2.9900 & 11.04 & 1.0033 & -     & 44.44 & 2.5861 & 2.8744 & \textbf{21.74} & 277.21 \\
% & Qwen2-1.5B      & \textbf{0.3946} & 2.0268 & \underline{63.21} & \textbf{0.4515} & 2.2946 & 55.56 & 1.4174 & 1.6468 & 14.05 & 185.22 \\
% & TinyLlama-1.1B  & 0.4281 & 2.0569 & 51.17 & 0.4716 & -     & 44.44 & 2.3999 & 2.5775 & \underline{19.73} & 198.72 \\
% & Llama-3.2-1B    & \underline{0.3979} & \underline{1.8683} & \textbf{63.79} & 0.6889 & \textbf{1.2530} & 42.22 & 1.5066 & 1.8534 & 11.71 & 280.32 \\
% & Llama-3.2-3B    & 0.6689 & 2.2351 & 40.80 & 0.4649 & 1.6299 & 44.44 & 1.2642 & \underline{0.7542} & 15.72 & \textbf{19.70} \\
% & Phi-3.5-mini    & 0.4047 & 2.3386 & 61.20 & \underline{0.4548} & 1.4096 & \underline{73.33} & \textbf{0.8760} & 0.8428 & 15.38 & \underline{56.75} \\
% & Qwen2.5-1.5B    & 0.5552 & 2.2458 & 62.88 & 0.9264 & 2.1170 & 55.56 & 1.3645 & 1.6254 & 15.72 & 72.20 \\
% \cmidrule{2-12}
% & Mean            & 0.605  & 2.150  & 52.2  & 0.602  & 1.654  & 55.00 & 1.489 & 1.552 & 16.43 & 143.23 \\
% \midrule

% \multirow{10}{*}{\makecell{\textbf{SLMs}\\(FS-3)}} 
% & gemma-2-2b-it   & 0.4816 & 1.6589 & 44.82 & 0.4883 & 1.653 & 53.3 & -     & -     & -     & - \\
% & Phi-3-mini-4k   & \underline{0.4114} & 1.6689 & 44.82 & \textbf{0.4515} & \textbf{0.574} & \underline{75.6} & \underline{0.880} & \textbf{0.535} & 19.4 & 54.983 \\
% & SmolLM-1.7B     & - & - & - & - & 0.740 & 53.3 & \textbf{0.870} & 0.582 & 15.4 & 18.972 \\
% & Qwen2-1.5B      & \underline{0.4114} & 1.6756 & \textbf{51.51} & \underline{0.4615} & \underline{0.661} & 57.8 & 0.883 & \textbf{0.535} & \underline{23.1} & 19.845 \\
% & TinyLlama-1.1B  & - & - & - & - & 0.820 & 44.4 & 2.933 & 3.043 & 14.4 & \textbf{17.902} \\
% & Llama-3.2-1B    & 0.4348 & 1.7324 & 49.83 & 0.5418 & 1.528 & 44.4 & 0.883 & \textbf{0.535} & 15.4 & \underline{18.472} \\
% & Llama-3.2-3B    & \underline{0.4114} & 1.7759 & \textbf{51.51} & 0.4682 & 1.014 & 42.2 & 1.194 & 1.117 & \textbf{24.1} & 19.270 \\
% & Phi-3.5-mini    & \underline{0.4114} & \textbf{1.4247} & \textbf{51.51} & \underline{0.4615} & 1.019 & \textbf{84.4} & 0.910 & \underline{0.548} & \textbf{24.1} & 32.941 \\
% & Qwen2.5-1.5B    & \textbf{0.3946} & \underline{1.4381} & \underline{37.12} & 0.7559 & 0.715 & 55.6 & 1.365 & 0.642 & 18.1 & \textbf{17.902} \\
% \cmidrule{2-12}
% & Mean            & 0.4224 & 1.6249 & 47.30 & 0.5184 & 0.969 & 56.8 & 1.240 & 0.942 & 19.2 & 25.036 \\
% \midrule

% \multirow{10}{*}{\makecell{\textbf{SLMs}\\(lora)}}
% & gemma-2-2b-it        & -      & -      & -    & 0.511 & \underline{0.723} & -     & 1.271 & 1.023 & \textbf{34.4} & \textbf{2.802} \\
% & Phi-3-mini-4k        & \underline{0.398} & 2.144 & \underline{62.2} & 0.522 & 0.966 & \textbf{68.9} & \textbf{0.809} & 0.712 & \underline{22.4} & 9.673 \\
% & SmolLM-1.7B          & 0.930  & 1.676  & 15.4 & 0.893 & 1.489 & 44.4  & 0.843 & \underline{0.539} & 16.1 & 18.868 \\
% & Qwen2-1.5B           & 0.428  & 1.522  & \underline{62.2} & \underline{0.472} & 0.903 & 55.6  & 0.923 & 0.967 & 18.7 & 5.211 \\
% & TinyLlama-1.1B       & \textbf{0.395} & \textbf{1.304} & \textbf{63.2} & \underline{0.472} & \textbf{0.667} & 55.6  & \underline{0.833} & 0.669 & 22.1 & 5.508 \\
% & Llama-3.2-1B         & 0.428  & 2.251  & 49.8 & 0.809 & 1.090 & 48.9  & 0.860 & \textbf{0.535} & 19.2 & 5.775 \\
% & Llama-3.2-3B         & 0.595  & 1.532  & 40.8 & \textbf{0.465} & 0.858 & 53.3  & 0.883 & \textbf{0.535} & 22.1 & \underline{3.640} \\
% & Phi-3.5-mini         & 0.485  & 1.548  & \underline{62.2} & 0.920 & 0.981 & \underline{62.2} & 0.880 & 0.659 & 19.4 & 12.091 \\
% & Qwen2.5-1.5B         & 0.866  & \underline{1.485} & 13.0 & 0.866 & 1.891 & 55.6  & 1.037 & 0.793 & 21.7 & 4.569 \\
% \cmidrule{2-12}
% & Mean                 & 0.566  & 1.683  & 46.1 & 0.659 & 1.063 & 55.6  & 0.927 & 0.715 & 21.8 & 7.571 \\

% % \midrule
% % \multirow{10}{*}{\makecell{\textbf{SLMs}\\(FT)}}
% % & gemma-2-2b-it        & \textbf{0.351} & \textbf{1.304} & 62.9 & \textbf{0.452} & 0.625 & 55.6 & 0.883 & \underline{0.535} & \underline{53.2} & \underline{2.147} \\
% % & Phi-3-mini-4k        & 0.398 & 1.535 & 62.9 & 0.468 & \underline{0.549} & \textbf{86.7} & \textbf{0.803} & 0.542 & 19.4 & 28.194 \\
% % & SmolLM-1.7B          & 0.732 & 2.993 & 18.1 & 1.672 & 14.757 & 43.2 & 1.997 & 0.686 & 16.0 & - \\
% % & Qwen2-1.5B           & 0.395 & \textbf{1.304} & \underline{63.2} & 0.478 & 0.820 & 55.6 & 1.050 & \underline{0.535} & 38.1 & 3.846 \\
% % & TinyLlama-1.1B       & 0.398 & \underline{1.331} & \underline{63.2} & \underline{0.455} & 0.675 & 44.4 & \underline{0.863} & \underline{0.535} & 38.1 & 2.312 \\
% % & Llama-3.2-1B         & 0.395 & 2.160 & \textbf{64.5} & 0.462 & 0.681 & 55.6 & - & - & 38.5 & 2.050 \\
% % & Llama-3.2-3B         & \underline{0.385} & \textbf{1.304} & 56.9 & \textbf{0.452} & 0.574 & - & 0.873 & \textbf{0.532} & \textbf{55.4} & \textbf{1.712} \\
% % & Phi-3.5-mini         & 0.535 & 1.512 & 61.2 & 0.508 & \textbf{0.450} & \underline{80.0} & 0.886 & 0.549 & 16.4 & 6.187 \\
% % & Qwen2.5-1.5B         & 0.682 & 1.446 & 39.6 & \underline{0.455} & 1.394 & 71.1 & 0.953 & 0.695 & 15.4 & 5.790 \\
% % \cmidrule{2-12}
% % & Mean                 & 0.474 & 1.655 & 54.7 & 0.600 & 2.281 & 61.5 & 1.038 & 0.576 & 32.3 & 6.530 \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}
